Automating Semantic Analysis of System Assurance Cases using Goal-directed ASP

Assurance cases offer a structured way to present arguments and evidence for certification of systems where safety and security are critical. However, creating and evaluating these assurance cases can be complex and challenging, even for systems of moderate complexity. Therefore, there is a growing need to develop new automation methods for these tasks. While most existing assurance case tools focus on automating structural aspects, they lack the ability to fully assess the semantic coherence and correctness of the assurance arguments. In prior work, we introduced the Assurance 2.0 framework that prioritizes the reasoning process, evidence utilization, and explicit delineation of counter-claims (defeaters) and counter-evidence. In this paper, we present our approach to enhancing Assurance 2.0 with semantic rule-based analysis capabilities using common-sense reasoning and answer set programming solvers, specifically s(CASP). By employing these analysis techniques, we examine the unique semantic aspects of assurance cases, such as logical consistency, adequacy, indefeasibility, etc. The application of these analyses provides both system developers and evaluators with increased confidence about the assurance case.

==> figures/Temp/OldIntroduction.tex <==
\section{Introduction}
\label{sec:introduction}

Certification of systems in regulated industries such as Aerospace, Nuclear, Automotive, etc., involves the verification of whether a particular system meets the relevant domain standards for specific concerns like security or safety. In recent years, there has been a rising interest in these domains regarding the development of ``assurance cases'' as an alternate means to establish credible confidence in claims made about a system's safety or security. Rather than the traditional approach of presenting a checklist of activities, assurance cases focus on creating a systematic argumentative record.  %These cases typically consist of claims defining the desired properties of the system's design and construction, evidence purportedly supporting the claims, and structured arguments demonstrating that the evidence sufficiently supports the claims. Rather than the traditional approach of presenting a checklist of activities, assurance cases focus on creating a systematic argumentative record. %Unlike the traditional approach of presenting a checklist of activities, assurance cases focus on creating a systematic argumentative record, making them a practical alternative for organizations seeking safety/security certification.

Essentially, assurance cases consist of claims about desired properties of the system's design and construction, evidence supporting the claims, and structured arguments that establish logical connections that the evidence sufficiently supports the claims. However, these cases for even moderately complex systems can become unwieldy, containing extensive hierarchical sets of arguments and evidence articulated in natural language. Authors and evaluators must therefore meticulously ensure the accuracy of the entire case to prevent the certification of unsafe or insecure systems, which unfortunately is a time-consuming and intellectually demanding task. Consequently, there is significant interest in implementing automation to both create and evaluate assurance cases, aiming to reduce human effort and bolster confidence in the cases. While most current assurance case tools and methodologies primarily concentrate on verifying the structural soundness of assurance cases, there is not adequate support to reason about the semantics or the meaning conveyed by the statements within the case.

%Fundamentally, a typical assurance case uses arguments to make logical connections between its top-level claim and its sub-claims or evidence. Unfortunately, assurance cases for even moderately complex systems can become large, comprising extensive sets of arguments and evidence expressed in natural language. Authors and evaluators must therefore diligently verify the correctness of the arguments and evidence to prevent certifying unsafe or insecure systems. This verification process is time-consuming, intellectually demanding, and prone to error. Hence, there is a great interest in Implementing automation to create and assess assurance cases to reduce human effort and enhance confidence in assurance cases. However, existing assurance case tools and approaches focus on checking the structural integrity of assurance cases, while there is not adequate support for reasoning about the semantics, i.e., the meaning of the words and statements used to describe the claims, arguments, and evidence, as well as verifying the logical relationships within the case. 
%Implementing rigorous automation for semantic analysis would reduce human effort and enhance confidence in assurance cases. 

%To address this challenge, we defined Consistent Logical Automated Reasoning for Integrated System Software Assurance (CLARISSA), a novel approach and associated tool suite to rigorously author and validate assurance cases~\cite[]}. One distinctive aspect of our approach, which we will explore in this paper, is the inclusion of semantic analysis capabilities by utilizing s(CASP), a solver for Constraints Answer Set Programs. Semantic analysis entails the examination of various properties specific to assurance cases, such as consistency, adequacy, indefeasibility, harmoniousness, and more. 

DARPA's Automated Rapid Certification of Software program sought to tackle the challenges associated with assurance case generation and validation.  As part of this initiative, we developed a comprehensive approach and tool suite named Consistent Logical Automated Reasoning for Integrated System Software Assurance (CLARISSA), which is founded on our assurance methodology called Assurance 2.0, and described by \cite{bloomfield2020assurance}. The uniqueness of Assurance 2.0 lies in its thorough deductive reasoning of claims, extensive exploration of doubts/objections, evaluation of evidence, and contextual interpretation of natural language assurance statements (see Section~\ref{sec:fram-assur-2.0}). While the comprehensive approach of CLARISSA is elaborated elsewhere, e.g., by \cite{finalCLARISSAReport, murugesan2023semantic}, this paper focuses on our approach to leveraging the power of common sense reasoning and answer set programming solvers, namely s(CASP), to automatically analyze the semantic aspects of the Assurance 2.0.

s(CASP), by \cite{scasp-iclp2018}, is a novel goal-oriented, non-monotonic reasoner capable of efficiently handling logical reasoning (see Section~\ref{sec:scasp-non-monotonic}) tasks essential for semantic analysis, which is central to our research. The goal-directed execution of s(CASP) % simulates human thinking by automating
automates commonsense reasoning based on general rules and exceptions (through default negation). I.e., it enables inferences to be drawn from a set of logical rules that formalize the assurance case. Additionally, s(CASP) performs \textit{deductive and abductive reasoning}, which is essential for proving whether a top-level claim can be deduced based on the arguments, evidence, and/or assumptions in assurance cases, and make it possible to define invariants (as \textit{global constraints}) that allows the analysis of scenarios that violate these invariants.

%\anitha{TODO: rephrase this paragraph about why Common sense reasoning, ASP and sCASP --JA: In fact this paragraph repeat what is said in Section~\ref{sec:scasp-non-monotonic} --I added some lines after next paragraph}

% The s(CASP) system is an answer set programming system for automating commonsense reasoning or human thinking. An assurance case captures human thinking and thus the s(CASP) system is ideal for checking the consistency of assurance cases.
% Our choice of s(CASP) is based on several reasons. Firstly, s(CASP) supports \textit{automated commonsense reasoning}, which enables inferences to be drawn from a set of predicates or knowledge in a manner similar to human reasoning. This feature is particularly well-suited for reasoning about assurance cases. Moreover, s(CASP) facilitates \textit{deductive and abductive reasoning}, which is essential for proving whether a top-level claim can be deduced based on the arguments, evidence, and assumptions in assurance cases.  Also, s(CASP) supports reasoning about \textit{global constraint}s and invariants, making it capable of analyzing scenarios that violate these constraints. Additionally, the top-down solving strategy employed by s(CASP) generates concise, human-understandable \textit{justifications}~\cite[]arias-justification}. These justifications play a crucial role in precisely identifying the reasons for assurance failure and resolving concerns. Furthermore, s(CASP) offers support for various forms of negation, which have diverse applications in assurance reasoning. For instance, we currently utilize \textit{default negation} to derive detailed justifications for why the top-level claim cannot be proven. Additionally, we are exploring the use of \textit{Negation as Failure}, which involves deriving negative conclusions from the absence of positive information, to automatically identify defeaters. Finally, s(CASP) possesses the ability to perform \textit{non-monotonic reasoning}, allowing for the revision of conclusions in light of new information. This feature is particularly valuable for incrementally assessing and improving the strength of assurance cases during the authoring process.



%In particular, Assurance 2.0 promotes the use of deductive reasoning, requiring that subclaims logically imply or entail the parent claim, which is a more robust approach compared to traditional inductive reasoning, where subclaims merely "suggest" the parent claim. Additionally, Assurance 2.0 mandates the \textit{Indefeasibility Criterion}, ensuring that all identified defeaters are addressed and that no credible doubts remain that could alter the conclusion. Furthermore, it mandates that natural language descriptions within the assurance case exhibit logical coherence, adequacy, harmoniousness, etc. While the comprehensive approach of CLARISSA is elaborated elsewhere~\cite[]}, this paper focuses on the utilization of s(CASP), a solver for Constraints Answer Set Programs, to automate the "semantic" analysis of Assurance 2.0, which would otherwise be intellectually demanding to perform.

The precursor to semantic analysis is rigorously identifying crucial lexical components within the assurance case statements. Intuitively, assurance statements describe the properties expressed by entities in a given environment. We leverage this understanding to establish minimal formalized semantics, identifying the words associated with objects, properties, and environments for each statement. Subsequently, we automatically translate this object-property-environment formalism of the entire assurance case into corresponding logical rules under  Answer Set Programming (ASP) semantics. Using various semantic properties of interest expressed as rules and queries, we use s(CASP) to provide the proof that these properties (represented as predicates) hold in the assurance case. % , that has been exported as Prolog predicates.

To the best of our knowledge, this methodology is not only the first attempt to tackle the automated semantic analysis of system assurance cases, it also establishes a new paradigm for explainable, knowledge-assisted assurance reasoning. This is thanks to the top-down solving strategy utilized by s(CASP), which produces concise and human-understandable justifications by \cite{arias-justification}. These justifications are essential to precisely identifying the reasons for the success (positive queries) or failure (negative queries) of the assurance, so that we can resolve the issues raised. % behind assurance success (positive queries), or failure (negative queries) so we can resolve the given concerns.
Furthermore, s(CASP) supports various forms of negation, each with unique applications in assurance reasoning. As we mention before, we use \textit{default negation} to derive detailed justifications for why a given  claim cannot be proven, while \textit{classical negation} can be used to impose specific restrictions (see the book by \cite{gelfond2014knowledge} for details).

%To the best of our knowledge, this methodology not only is the first attempt to address the automated semantic analysis of system assurance cases but also establishes a new paradigm for explainable knowledge-assisted assurance reasoning, because, the top-down solving strategy employed by s(CASP) generates concise, human-understandable \textit{justifications}~\cite[]arias-justification}. These justifications play a crucial role in precisely identifying the reasons for assurance failure and resolving concerns. Furthermore, s(CASP) supports several forms of negation, which have diverse applications in assurance reasoning. We also utilize \textit{default negation} to derive detailed justifications for why the top-level claim cannot be proven, while \textit{classical negation} could be used to impose additional invariants.
  
In the rest of the paper, we describe this approach in depth using the ArduCopter system, an open-source platform (see Section~\ref{sec:case-study:-arduc}), as an illustrative example to demonstrate the feasibility of our approach by highlighting the following contributions:
\begin{itemize}

\item Methodically identify and capture the vocabulary within each assurance case statement that contributes to the lexical significance of the assurance case. The main steps of this methodology are outlined in Section~\ref{sec:semant-analys-appr}. 

\item Systematically translate the assurance case into a logic program in ASP  that is amenable for analysis using s(CASP). To facilitate this, we have enhanced the ASCE tool with a plugin that captures the vocabulary and automatically transforms the use case into logical notation. The new plugin is described in Section~\ref{sec:form-assur-stat},  and the transformation mapping is explained in Section~\ref{sec:transf-logic-notat}.
    
\item Identify and formalize properties that are unique and essential for assessing the semantic rigor of assurance cases. These properties are elaborated in Section~\ref{sec:semant-prop-defin}. % and formally define them. %.Identify and formally define assurance case-centric semantic properties aimed at strengthening the rigor of the analysis of these cases. 

\item Leverage the capabilities of s(CASP) tool to analyze semantic properties within the assurance case, as described in  Section~\ref{sec:semant-analys-using}. In particular, our use of \textit{Negation as Failure} involves deriving negative conclusions from the absence of positive information, to automatically identify defeaters. Additionally, s(CASP) possesses the ability to perform \textit{non-monotonic reasoning} that allows revision of conclusions in light of new information. This feature is particularly valuable for incrementally assessing and improving the strength of assurance cases during the authoring process.

%\item Finally, in Section~\ref{sec:semant-analys-using} we describe how the s(CASP) tool is leveraged to analyze semantic properties within the assurance case. In particular, we are exploring the use of \textit{Negation as Failure}, which involves deriving negative conclusions from the absence of positive information, to automatically identify defeaters. Additionally, s(CASP) possesses the ability to perform \textit{non-monotonic reasoning}, which allows revision of conclusions in light of new information. This feature is particularly valuable for incrementally assessing and improving the strength of assurance cases during the authoring process.
\end{itemize}


%\anitha{TO DO : paragraph to say something about: to the best of our knowledge this is the first time this approach has been used to address this problem; establishing a new paradigm for explainable knowledge-assisted assurance reasoning. --JA: Agree}



% {\color{red} NOT NEEDED --already pointed in itemize
%   The structure of this paper is as follows. Section 2 outlines the foundation of Assurance 2.0 and offers a concise overview of the Arducopter case example along with its assurance case. In Section 3 describes our methodology. In Section 4, provides a brief introduction of s(Casp) followed by details of the various semantic analyses conducted. Finally, Section 5 wraps up with concluding remarks, insights gained, and avenues for future research.
% }







%One distinctive aspect of our approach, which we will explore in this paper, is the inclusion of semantic analysis capabilities by utilizing s(CASP), a solver for Constraints Answer Set Programs. Semantic analysis entails the examination of various properties specific to assurance cases, such as consistency, adequacy, indefeasibility, harmoniousness, and more. 


%To address this challenge, we defined Consistent Logical Automated Reasoning for Integrated System Software Assurance (CLARISSA), a novel approach and associated tool suite to rigorously author and validate assurance cases~\cite[]}. It is based on Assurance 2.0 methodology, a modern framework to effectively capture assurance cases.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Main"
%%% End:
